On the use of dielectric elements in axion searches with microwave resonant cavities

This study explores the primary effects of dielectric materials in a resonant cavity-based search for axion dark matter. While dielectrics prove beneficial in numerous cases, their incorporation may lead to less-than-optimal performance, especially for the lowest TM mode. Additionally, the stronger confinement of the electric field inside the dielectrics can exacerbate mode mixings, in particular for higher-order modes. Case studies have been carried out using a combination of analytical solutions and numerical simulations. The findings indicate dielectric cavities employing the $\text{TM}_{010}$ mode experience a significant reduction in sensitivity when compared to a similar search conducted in a cavity at equivalent frequency using no dielectrics.

==> format.tex <==
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{epstopdf}
\epstopdfsetup{verbose=false}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{enumitem}
\usepackage{color}
\usepackage{multirow}
\usepackage[colorlinks=true,linkcolor=blue,allcolors=blue]{hyperref} % for links 
%\usepackage[caption=false]{subfig}
%\captionsetup[subfigure]{labelformat=brace}
%\usepackage{biblatex}

\usepackage{xcolor}

%Get quotes to open correctly
\usepackage [autostyle, english = american]{csquotes}
\MakeOuterQuote{"}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% packages
\usepackage{mathtools} 	%% because math++
\usepackage{comment} 	%% block comments 
\usepackage{multirow}	%% for longer eq.
%\usepackage{gensymb}
\usepackage{epstopdf}
\usepackage[]{siunitx}  %% because of \mu vs \si{\micro}
\sisetup{
  per-mode=symbol,
  fraction-function=\tfrac
}
\DeclareSIUnit\sample{S}
\DeclareSIUnit\bits{bits}
\usepackage{amsmath} 
\usepackage{lineno} 	%% for line numbers
%%%%%% patch lineno spacing around ams math environs, %http://phaseportrait.blogspot.com/2007/08/lineno-and-amsmath-compatibility.html
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}% 
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}
%%%%% /patched
\usepackage{xspace} 	%% for commands that don't eat spaces afterwards
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% shortcuts for everywhere
\newcommand{\znbb} {$0\nu\!\beta\!\beta$\xspace}
\newcommand{\tnbb} {$2\nu\!\beta\!\beta$\xspace}
\newcommand{\otsx} {$^{136}\mathrm{Xe}$\xspace}

\newcommand{\sep}{, } %% keyword separator
%\newcommand{\Efield} {380~V/cm\xspace}

\newcommand{\cudepth}{\SI{125}{\micro\metre}\xspace}
\newcommand{\cavlength}{\SI{25.4}{\cm}\xspace}
\newcommand{\cavdiameter}{\SI{10.2}{\cm}\xspace}
\newcommand{\cavfullvolume}{\SI{2}{\litre}\xspace}
\newcommand{\cavaxionvolume}{\SI{1.545}{\litre}\xspace}
\newcommand{\roddiameter}{\SI{5.1}{\cm}\xspace}
\newcommand{\rodgap}{$\sim$\SI{250}{\micro\metre}\xspace}
\newcommand{\magfield}{\SI{8}{T}\xspace}
\newcommand{\jpaheight}{$\sim$\SI{60}{\cm}\xspace}
\newcommand{\frange}{4.46-\SI{4.52}{\GHz}\xspace}
\newcommand{\fwindow}{\SI{60}{\MHz}}
\newcommand{\origdays}{100ish \fxnote{fix}}
\newcommand{\seglen}{\SI{10}{\ms\xspace}}

\newcommand{\PIIaEpsilon}{\SI{50}{\percent\xspace}}
\newcommand{\PIIbEpsilon}{\SI{80}{\percent\xspace}}

\newcommand{\mjcom}[1]{\xspace{\color{red} MJ: #1}\xspace}

\newcommand{\basetemp}{61.0$\pm$\SI{0.1}{mK}}

\newcommand{\chirfl}{$\left| \chi_{rfl} \right|^{2}$\xspace}
\newcommand{\axpwr}{$P_\text{ax}$\xspace}

%Phase names
\newcommand{\PI}{Phase I\xspace}
\newcommand{\PII}{Phase II\xspace}
\newcommand{\PIIa}{Phase IIa\xspace}
\newcommand{\PIIb}{Phase IIb\xspace}

\newcommand{\SQZ}{SQZ\xspace}
\newcommand{\AMP}{AMP\xspace}
\newcommand{\TMC}{$T_\text{mc}$\xspace}
\newcommand{\gagg}{$g_{\alpha\gamma\gamma}$\xspace}
\newcommand{\ggam}{$g_{\gamma}$\xspace}
\newcommand{\daqenhance}{$\sim$1.6\xspace}

\newcommand{\axcoup}{$g_{\alpha\gamma\gamma}$\xspace}

%% trim toc
\setcounter{tocdepth}{2}
\makeatletter
\renewcommand\tableofcontents{%
    \@starttoc{toc}%
}
\makeatother



%%% revision marking
\newif\ifshowchanges
\showchangesfalse
% \showchangesfalse % false show   changes

\newcommand{\vo}[1]{}
\newcommand{\vf}[1]{{{#1}}}
\newcommand{\fixme}[1]{{\textcolor{red}{#1}}}

\ifshowchanges
\usepackage{soul}
\soulregister\cite7
\soulregister\ref7
	\renewcommand{\vo}[1]{{\textcolor{red}{\st{#1}}}}
    \renewcommand{\vf}[1]{\textcolor{cyan}{{#1}}}
\fi

%\usepackage{caption}
%\usepackage{subcaption}
\usepackage{soul}
\usepackage{fixme}
%\fxsetup{status=draft,theme=color}
\fxsetup{status=draft,theme=color, layout=inline}
\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
